Constraints on the CKM angle $\gamma$ from $B^\pm\to Dh^\pm$ decays using $D\rightarrow h^\pm h^{\prime\mp}\pi^0$ final states

A data sample collected with the LHCb detector corresponding to an integrated luminosity of 9 fb$^{-1}$ is used to measure eleven $CP$ violation observables in $B^\pm\to Dh^\pm$ decays, where $h$ is either a kaon or a pion. The neutral $D$ meson decay is reconstructed in the three-body final states: $K^\pm\pi^\mp\pi^0$}; $\pi^+\pi^-\pi^0$; $K^+K^-\pi^0$ and the suppressed $\pi^\pm K^\mp\pi^0$ combination. The mode where a large $CP$ asymmetry is expected, $B^\pm\to [\pi^\pm K^\mp\pi^0]_DK^\pm$, is observed with a significance greater than seven standard deviations. The ratio of the partial width of this mode relative to that of the favoured mode, $B^\pm\to [K^\pm\pi^\mp\pi^0]_D K^\pm$, is $R_{{\rm ADS}(K)} = (1.27\pm0.16\pm0.02)\times 10^{-2}$. Evidence for a large $CP$ asymmetry is also seen: $A_{{\rm ADS}(K)} = -0.38\pm0.12\pm0.02$. Constraints on the CKM angle $\gamma$ are calculated from the eleven reported observables.

==> Authorship_LHCb-PAPER-2021-036-arXiv.tex <==
LHCb collaboration:
R. Aaij,
A.S.W. Abdelmotteleb,
C. Abell{\'a}n Beteta,
F. Abudin{\'e}n,
T. Ackernley,
B. Adeva,
M. Adinolfi,
H. Afsharnia,
C. Agapopoulou,
C.A. Aidala,
S. Aiola,
Z. Ajaltouni,
S. Akar,
J. Albrecht,
F. Alessio,
M. Alexander,
A. Alfonso Albero,
Z. Aliouche,
G. Alkhazov,
P. Alvarez Cartelle,
S. Amato,
J.L. Amey,
Y. Amhis,
L. An,
L. Anderlini,
M. Andersson,
A. Andreianov,
M. Andreotti,
F. Archilli,
A. Artamonov,
M. Artuso,
K. Arzymatov,
E. Aslanides,
M. Atzeni,
B. Audurier,
S. Bachmann,
M. Bachmayer,
J.J. Back,
P. Baladron Rodriguez,
V. Balagura,
W. Baldini,
J. Baptista de Souza Leite,
M. Barbetti,
R.J. Barlow,
S. Barsuk,
W. Barter,
M. Bartolini,
F. Baryshnikov,
J.M. Basels,
G. Bassi,
B. Batsukh,
A. Battig,
A. Bay,
A. Beck,
M. Becker,
F. Bedeschi,
I. Bediaga,
A. Beiter,
V. Belavin,
S. Belin,
V. Bellee,
K. Belous,
I. Belov,
I. Belyaev,
G. Bencivenni,
E. Ben-Haim,
A. Berezhnoy,
R. Bernet,
D. Berninghoff,
H.C. Bernstein,
C. Bertella,
A. Bertolin,
C. Betancourt,
F. Betti,
Ia. Bezshyiko,
S. Bhasin,
J. Bhom,
L. Bian,
M.S. Bieker,
N.V. Biesuz,
S. Bifani,
P. Billoir,
A. Biolchini,
M. Birch,
F.C.R. Bishop,
A. Bitadze,
A. Bizzeti,
M. Bj{\o}rn,
M.P. Blago,
T. Blake,
F. Blanc,
S. Blusk,
D. Bobulska,
J.A. Boelhauve,
O. Boente Garcia,
T. Boettcher,
A. Boldyrev,
A. Bondar,
N. Bondar,
S. Borghi,
M. Borisyak,
M. Borsato,
J.T. Borsuk,
S.A. Bouchiba,
T.J.V. Bowcock,
A. Boyer,
C. Bozzi,
M.J. Bradley,
S. Braun,
A. Brea Rodriguez,
J. Brodzicka,
A. Brossa Gonzalo,
D. Brundu,
A. Buonaura,
L. Buonincontri,
A.T. Burke,
C. Burr,
A. Bursche,
A. Butkevich,
J.S. Butter,
J. Buytaert,
W. Byczynski,
S. Cadeddu,
H. Cai,
R. Calabrese,
L. Calefice,
S. Cali,
R. Calladine,
M. Calvi,
M. Calvo Gomez,
P. Camargo Magalhaes,
P. Campana,
A.F. Campoverde Quezada,
S. Capelli,
L. Capriotti,
A. Carbone,
G. Carboni,
R. Cardinale,
A. Cardini,
I. Carli,
P. Carniti,
L. Carus,
K. Carvalho Akiba,
A. Casais Vidal,
R. Caspary,
G. Casse,
M. Cattaneo,
G. Cavallero,
S. Celani,
J. Cerasoli,
D. Cervenkov,
A.J. Chadwick,
M.G. Chapman,
M. Charles,
Ph. Charpentier,
G. Chatzikonstantinidis,
C.A. Chavez Barajas,
M. Chefdeville,
C. Chen,
S. Chen,
A. Chernov,
V. Chobanova,
S. Cholak,
M. Chrzaszcz,
A. Chubykin,
V. Chulikov,
P. Ciambrone,
M.F. Cicala,
X. Cid Vidal,
G. Ciezarek,
P.E.L. Clarke,
M. Clemencic,
H.V. Cliff,
J. Closier,
J.L. Cobbledick,
V. Coco,
J.A.B. Coelho,
J. Cogan,
E. Cogneras,
L. Cojocariu,
P. Collins,
T. Colombo,
L. Congedo,
A. Contu,
N. Cooke,
G. Coombs,
I. Corredoira ,
G. Corti,
C.M. Costa Sobral,
B. Couturier,
D.C. Craik,
J. Crkovsk\'{a},
M. Cruz Torres,
R. Currie,
C.L. Da Silva,
S. Dadabaev,
L. Dai,
E. Dall'Occo,
J. Dalseno,
C. D'Ambrosio,
A. Danilina,
P. d'Argent,
A. Dashkina,
J.E. Davies,
A. Davis,
O. De Aguiar Francisco,
K. De Bruyn,
S. De Capua,
M. De Cian,
E. De Lucia,
J.M. De Miranda,
L. De Paula,
M. De Serio,
D. De Simone,
P. De Simone,
F. De Vellis,
J.A. de Vries,
C.T. Dean,
F. Debernardis,
D. Decamp,
V. Dedu,
L. Del Buono,
B. Delaney,
H.-P. Dembinski,
A. Dendek,
V. Denysenko,
D. Derkach,
O. Deschamps,
F. Desse,
F. Dettori,
B. Dey,
A. Di Cicco,
P. Di Nezza,
S. Didenko,
L. Dieste Maronas,
H. Dijkstra,
V. Dobishuk,
C. Dong,
A.M. Donohoe,
F. Dordei,
A.C. dos Reis,
L. Douglas,
A. Dovbnya,
A.G. Downes,
M.W. Dudek,
L. Dufour,
V. Duk,
P. Durante,
J.M. Durham,
D. Dutta,
A. Dziurda,
A. Dzyuba,
S. Easo,
U. Egede,
V. Egorychev,
S. Eidelman,
S. Eisenhardt,
S. Ek-In,
L. Eklund,
S. Ely,
A. Ene,
E. Epple,
S. Escher,
J. Eschle,
S. Esen,
T. Evans,
L.N. Falcao,
Y. Fan,
B. Fang,
S. Farry,
D. Fazzini,
M. F{\'e}o,
A. Fernandez Prieto,
A.D. Fernez,
F. Ferrari,
L. Ferreira Lopes,
F. Ferreira Rodrigues,
S. Ferreres Sole,
M. Ferrillo,
M. Ferro-Luzzi,
S. Filippov,
R.A. Fini,
M. Fiorini,
M. Firlej,
K.M. Fischer,
D.S. Fitzgerald,
C. Fitzpatrick,
T. Fiutowski,
A. Fkiaras,
F. Fleuret,
M. Fontana,
F. Fontanelli,
R. Forty,
D. Foulds-Holt,
V. Franco Lima,
M. Franco Sevilla,
M. Frank,
E. Franzoso,
G. Frau,
C. Frei,
D.A. Friday,
J. Fu,
Q. Fuehring,
E. Gabriel,
G. Galati,
A. Gallas Torreira,
D. Galli,
S. Gambetta,
Y. Gan,
M. Gandelman,
P. Gandini,
Y. Gao,
M. Garau,
L.M. Garcia Martin,
P. Garcia Moreno,
J. Garc{\'\i}a Pardi{\~n}as,
B. Garcia Plana,
F.A. Garcia Rosales,
L. Garrido,
C. Gaspar,
R.E. Geertsema,
D. Gerick,
L.L. Gerken,
E. Gersabeck,
M. Gersabeck,
T. Gershon,
D. Gerstel,
L. Giambastiani,
V. Gibson,
H.K. Giemza,
A.L. Gilman,
M. Giovannetti,
A. Giovent{\`u},
P. Gironella Gironell,
C. Giugliano,
K. Gizdov,
E.L. Gkougkousis,
V.V. Gligorov,
C. G{\"o}bel,
E. Golobardes,
D. Golubkov,
A. Golutvin,
A. Gomes,
S. Gomez Fernandez,
F. Goncalves Abrantes,
M. Goncerz,
G. Gong,
P. Gorbounov,
I.V. Gorelov,
C. Gotti,
E. Govorkova,
J.P. Grabowski,
T. Grammatico,
L.A. Granado Cardoso,
E. Graug{\'e}s,
E. Graverini,
G. Graziani,
A. Grecu,
L.M. Greeven,
N.A. Grieser,
L. Grillo,
S. Gromov,
B.R. Gruberg Cazon,
C. Gu,
M. Guarise,
M. Guittiere,
P. A. G{\"u}nther,
E. Gushchin,
A. Guth,
Y. Guz,
T. Gys,
T. Hadavizadeh,
G. Haefeli,
C. Haen,
J. Haimberger,
T. Halewood-leagas,
P.M. Hamilton,
J.P. Hammerich,
Q. Han,
X. Han,
T.H. Hancock,
E.B. Hansen,
S. Hansmann-Menzemer,
N. Harnew,
T. Harrison,
C. Hasse,
M. Hatch,
J. He,
M. Hecker,
K. Heijhoff,
K. Heinicke,
R.D.L. Henderson,
A.M. Hennequin,
K. Hennessy,
L. Henry,
J. Heuel,
A. Hicheur,
D. Hill,
M. Hilton,
S.E. Hollitt,
R. Hou,
Y. Hou,
J. Hu,
J. Hu,
W. Hu,
X. Hu,
W. Huang,
X. Huang,
W. Hulsbergen,
R.J. Hunter,
M. Hushchyn,
D. Hutchcroft,
D. Hynds,
P. Ibis,
M. Idzik,
D. Ilin,
P. Ilten,
A. Inglessi,
A. Ishteev,
K. Ivshin,
R. Jacobsson,
H. Jage,
S. Jakobsen,
E. Jans,
B.K. Jashal,
A. Jawahery,
V. Jevtic,
X. Jiang,
M. John,
D. Johnson,
C.R. Jones,
T.P. Jones,
B. Jost,
N. Jurik,
S. Kandybei,
Y. Kang,
M. Karacson,
M. Karpov,
J.W. Kautz,
F. Keizer,
D.M. Keller,
M. Kenzie,
T. Ketel,
B. Khanji,
A. Kharisova,
S. Kholodenko,
T. Kirn,
V.S. Kirsebom,
O. Kitouni,
S. Klaver,
N. Kleijne,
K. Klimaszewski,
M.R. Kmiec,
S. Koliiev,
A. Kondybayeva,
A. Konoplyannikov,
P. Kopciewicz,
R. Kopecna,
P. Koppenburg,
M. Korolev,
I. Kostiuk,
O. Kot,
S. Kotriakhova,
P. Kravchenko,
L. Kravchuk,
R.D. Krawczyk,
M. Kreps,
F. Kress,
S. Kretzschmar,
P. Krokovny,
W. Krupa,
W. Krzemien,
J. Kubat,
M. Kucharczyk,
V. Kudryavtsev,
H.S. Kuindersma,
G.J. Kunde,
T. Kvaratskheliya,
D. Lacarrere,
G. Lafferty,
A. Lai,
A. Lampis,
D. Lancierini,
J.J. Lane,
R. Lane,
G. Lanfranchi,
C. Langenbruch,
J. Langer,
O. Lantwin,
T. Latham,
F. Lazzari,
R. Le Gac,
S.H. Lee,
R. Lef{\`e}vre,
A. Leflat,
S. Legotin,
O. Leroy,
T. Lesiak,
B. Leverington,
H. Li,
P. Li,
S. Li,
Y. Li,
Y. Li,
Z. Li,
X. Liang,
T. Lin,
R. Lindner,
V. Lisovskyi,
R. Litvinov,
G. Liu,
H. Liu,
Q. Liu,
S. Liu,
A. Lobo Salvia,
A. Loi,
J. Lomba Castro,
I. Longstaff,
J.H. Lopes,
S. L{\'o}pez Soli{\~n}o,
G.H. Lovell,
Y. Lu,
C. Lucarelli,
D. Lucchesi,
S. Luchuk,
M. Lucio Martinez,
V. Lukashenko,
Y. Luo,
A. Lupato,
E. Luppi,
O. Lupton,
A. Lusiani,
X. Lyu,
L. Ma,
R. Ma,
S. Maccolini,
F. Machefert,
F. Maciuc,
V. Macko,
P. Mackowiak,
S. Maddrell-Mander,
L.R. Madhan Mohan,
O. Maev,
A. Maevskiy,
M.W. Majewski,
J.J. Malczewski,
S. Malde,
B. Malecki,
A. Malinin,
T. Maltsev,
H. Malygina,
G. Manca,
G. Mancinelli,
D. Manuzzi,
D. Marangotto,
J. Maratas,
J.F. Marchand,
U. Marconi,
S. Mariani,
C. Marin Benito,
M. Marinangeli,
J. Marks,
A.M. Marshall,
P.J. Marshall,
G. Martelli,
G. Martellotti,
L. Martinazzoli,
M. Martinelli,
D. Martinez Santos,
F. Martinez Vidal,
A. Massafferri,
M. Materok,
R. Matev,
A. Mathad,
V. Matiunin,
C. Matteuzzi,
K.R. Mattioli,
A. Mauri,
E. Maurice,
J. Mauricio,
M. Mazurek,
M. McCann,
L. Mcconnell,
T.H. Mcgrath,
N.T. Mchugh,
A. McNab,
R. McNulty,
J.V. Mead,
B. Meadows,
G. Meier,
D. Melnychuk,
S. Meloni,
M. Merk,
A. Merli,
L. Meyer Garcia,
M. Mikhasenko,
D.A. Milanes,
E. Millard,
M. Milovanovic,
M.-N. Minard,
A. Minotti,
L. Minzoni,
S.E. Mitchell,
B. Mitreska,
D.S. Mitzel,
A. M{\"o}dden ,
R.A. Mohammed,
R.D. Moise,
S. Mokhnenko,
T. Momb{\"a}cher,
I.A. Monroy,
S. Monteil,
M. Morandin,
G. Morello,
M.J. Morello,
J. Moron,
A.B. Morris,
A.G. Morris,
R. Mountain,
H. Mu,
F. Muheim,
M. Mulder,
D. M{\"u}ller,
K. M{\"u}ller,
C.H. Murphy,
D. Murray,
R. Murta,
P. Muzzetto,
P. Naik,
T. Nakada,
R. Nandakumar,
T. Nanut,
I. Nasteva,
M. Needham,
N. Neri,
S. Neubert,
N. Neufeld,
R. Newcombe,
E.M. Niel,
S. Nieswand,
N. Nikitin,
N.S. Nolte,
C. Normand,
C. Nunez,
A. Oblakowska-Mucha,
V. Obraztsov,
T. Oeser,
D.P. O'Hanlon,
S. Okamura,
R. Oldeman,
F. Oliva,
M.E. Olivares,
C.J.G. Onderwater,
R.H. O'Neil,
J.M. Otalora Goicochea,
T. Ovsiannikova,
P. Owen,
A. Oyanguren,
K.O. Padeken,
B. Pagare,
P.R. Pais,
T. Pajero,
A. Palano,
M. Palutan,
Y. Pan,
G. Panshin,
A. Papanestis,
M. Pappagallo,
L.L. Pappalardo,
C. Pappenheimer,
W. Parker,
C. Parkes,
B. Passalacqua,
G. Passaleva,
A. Pastore,
M. Patel,
C. Patrignani,
C.J. Pawley,
A. Pearce,
A. Pellegrino,
M. Pepe Altarelli,
S. Perazzini,
D. Pereima,
A. Pereiro Castro,
P. Perret,
M. Petric,
K. Petridis,
A. Petrolini,
A. Petrov,
S. Petrucci,
M. Petruzzo,
T.T.H. Pham,
A. Philippov,
R. Piandani,
L. Pica,
M. Piccini,
B. Pietrzyk,
G. Pietrzyk,
M. Pili,
D. Pinci,
F. Pisani,
M. Pizzichemi,
Resmi  P.K,
V. Placinta,
J. Plews,
M. Plo Casasus,
F. Polci,
M. Poli Lener,
M. Poliakova,
A. Poluektov,
N. Polukhina,
I. Polyakov,
E. Polycarpo,
S. Ponce,
D. Popov,
S. Popov,
S. Poslavskii,
K. Prasanth,
L. Promberger,
C. Prouve,
V. Pugatch,
V. Puill,
H. Pullen,
G. Punzi,
H. Qi,
W. Qian,
N. Qin,
R. Quagliani,
N.V. Raab,
R.I. Rabadan Trejo,
B. Rachwal,
J.H. Rademacker,
M. Rama,
M. Ramos Pernas,
M.S. Rangel,
F. Ratnikov,
G. Raven,
M. Reboud,
F. Redi,
F. Reiss,
C. Remon Alepuz,
Z. Ren,
V. Renaudin,
R. Ribatti,
S. Ricciardi,
K. Rinnert,
P. Robbe,
G. Robertson,
A.B. Rodrigues,
E. Rodrigues,
J.A. Rodriguez Lopez,
E.R.R. Rodriguez Rodriguez,
A. Rollings,
P. Roloff,
V. Romanovskiy,
M. Romero Lamas,
A. Romero Vidal,
J.D. Roth,
M. Rotondo,
M.S. Rudolph,
T. Ruf,
R.A. Ruiz Fernandez,
J. Ruiz Vidal,
A. Ryzhikov,
J. Ryzka,
J.J. Saborido Silva,
N. Sagidova,
N. Sahoo,
B. Saitta,
M. Salomoni,
C. Sanchez Gras,
R. Santacesaria,
C. Santamarina Rios,
M. Santimaria,
E. Santovetti,
D. Saranin,
G. Sarpis,
M. Sarpis,
A. Sarti,
C. Satriano,
A. Satta,
M. Saur,
D. Savrina,
H. Sazak,
L.G. Scantlebury Smead,
A. Scarabotto,
S. Schael,
S. Scherl,
M. Schiller,
H. Schindler,
M. Schmelling,
B. Schmidt,
S. Schmitt,
O. Schneider,
A. Schopper,
M. Schubiger,
S. Schulte,
M.H. Schune,
R. Schwemmer,
B. Sciascia,
S. Sellam,
A. Semennikov,
M. Senghi Soares,
A. Sergi,
N. Serra,
L. Sestini,
A. Seuthe,
Y. Shang,
D.M. Shangase,
M. Shapkin,
I. Shchemerov,
L. Shchutska,
T. Shears,
L. Shekhtman,
Z. Shen,
S. Sheng,
V. Shevchenko,
E.B. Shields,
Y. Shimizu,
E. Shmanin,
J.D. Shupperd,
B.G. Siddi,
R. Silva Coutinho,
G. Simi,
S. Simone,
N. Skidmore,
T. Skwarnicki,
M.W. Slater,
I. Slazyk,
J.C. Smallwood,
J.G. Smeaton,
A. Smetkina,
E. Smith,
M. Smith,
A. Snoch,
L. Soares Lavra,
M.D. Sokoloff,
F.J.P. Soler,
A. Solovev,
I. Solovyev,
F.L. Souza De Almeida,
B. Souza De Paula,
B. Spaan,
E. Spadaro Norella,
P. Spradlin,
F. Stagni,
M. Stahl,
S. Stahl,
S. Stanislaus,
O. Steinkamp,
O. Stenyakin,
H. Stevens,
S. Stone,
D. Strekalina,
F. Suljik,
J. Sun,
L. Sun,
Y. Sun,
P. Svihra,
P.N. Swallow,
K. Swientek,
A. Szabelski,
T. Szumlak,
M. Szymanski,
S. Taneja,
A.R. Tanner,
M.D. Tat,
A. Terentev,
F. Teubert,
E. Thomas,
D.J.D. Thompson,
K.A. Thomson,
H. Tilquin,
V. Tisserand,
S. T'Jampens,
M. Tobin,
L. Tomassetti,
X. Tong,
D. Torres Machado,
D.Y. Tou,
E. Trifonova,
S.M. Trilov,
C. Trippl,
G. Tuci,
A. Tully,
N. Tuning,
A. Ukleja,
D.J. Unverzagt,
E. Ursov,
A. Usachov,
A. Ustyuzhanin,
U. Uwer,
A. Vagner,
V. Vagnoni,
A. Valassi,
G. Valenti,
N. Valls Canudas,
M. van Beuzekom,
M. Van Dijk,
H. Van Hecke,
E. van Herwijnen,
M. van Veghel,
R. Vazquez Gomez,
P. Vazquez Regueiro,
C. V{\'a}zquez Sierra,
S. Vecchi,
J.J. Velthuis,
M. Veltri,
A. Venkateswaran,
M. Veronesi,
M. Vesterinen,
D.  Vieira,
M. Vieites Diaz,
H. Viemann,
X. Vilasis-Cardona,
E. Vilella Figueras,
A. Villa,
P. Vincent,
F.C. Volle,
D. Vom Bruch,
A. Vorobyev,
V. Vorobyev,
N. Voropaev,
K. Vos,
R. Waldi,
J. Walsh,
C. Wang,
J. Wang,
J. Wang,
J. Wang,
J. Wang,
M. Wang,
R. Wang,
Y. Wang,
Z. Wang,
Z. Wang,
Z. Wang,
J.A. Ward,
N.K. Watson,
S.G. Weber,
D. Websdale,
C. Weisser,
B.D.C. Westhenry,
D.J. White,
M. Whitehead,
A.R. Wiederhold,
D. Wiedner,
G. Wilkinson,
M. K. Wilkinson,
I. Williams,
M. Williams,
M.R.J. Williams,
F.F. Wilson,
W. Wislicki,
M. Witek,
L. Witola,
G. Wormser,
S.A. Wotton,
H. Wu,
K. Wyllie,
Z. Xiang,
D. Xiao,
Y. Xie,
A. Xu,
J. Xu,
L. Xu,
M. Xu,
Q. Xu,
Z. Xu,
Z. Xu,
D. Yang,
S. Yang,
Y. Yang,
Z. Yang,
Z. Yang,
Y. Yao,
L.E. Yeomans,
H. Yin,
J. Yu,
X. Yuan,
O. Yushchenko,
E. Zaffaroni,
M. Zavertyaev,
M. Zdybal,
O. Zenaiev,
M. Zeng,
D. Zhang,
L. Zhang,
S. Zhang,
S. Zhang,
Y. Zhang,
Y. Zhang,
A. Zharkova,
A. Zhelezov,
Y. Zheng,
T. Zhou,
X. Zhou,
Y. Zhou,
V. Zhovkovska,
X. Zhu,
X. Zhu,
Z. Zhu,
V. Zhukov,
J.B. Zonneveld,
Q. Zou,
S. Zucchelli,
D. Zuliani,
G. Zunica
